Reversible Sessions Using Monitors

Much research has studied foundations for correct and reliable communication-centric systems. A salient approach to correctness uses session types to enforce structured communications; a recent approach to reliability uses reversible actions as a way of reacting to unanticipated events or failures. This note develops a simple observation: the machinery required to define asynchronous semantics and monitoring can also support reversible protocols. We propose a process framework of session communication in which monitors support reversibility. A key novelty in our approach are session types with present and past, which allow us to streamline the semantics of reversible actions.

==> eptcsdata.tex <==
\providecommand{\firstpage}{56}
\providecommand{\publicationstatus}{D. Orchard and N. Yoshida (Eds.): Programming Language Approaches to \\ Concurrency- and Communication-Centric Software (PLACES 2016).\\
EPTCS 211, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.211.6}{10.4204/EPTCS.211.6}}

